Robust Orthogonal Complement Principal Component Analysis

Recently, the robustification of principal component analysis has attracted lots of attention from statisticians, engineers and computer scientists. In this work we study the type of outliers that are not necessarily apparent in the original observation space but can seriously affect the principal subspace estimation. Based on a mathematical formulation of such transformed outliers, a novel robust orthogonal complement principal component analysis (ROC-PCA) is proposed. The framework combines the popular sparsity-enforcing and low rank regularization techniques to deal with row-wise outliers as well as element-wise outliers. A non-asymptotic oracle inequality guarantees the accuracy and high breakdown performance of ROC-PCA in finite samples. To tackle the computational challenges, an efficient algorithm is developed on the basis of Stiefel manifold optimization and iterative thresholding. Furthermore, a batch variant is proposed to significantly reduce the cost in ultra high dimensions. The paper also points out a pitfall of a common practice of SVD reduction in robust PCA. Experiments show the effectiveness and efficiency of ROC-PCA in both synthetic and real data.

==> algdescription.tex <==
% \IncMargin{1em}
% \linesnumbered
\restylealgo{ruled}
\begin{algorithm}
    \label{alg:ROCPCAAlgorithm}

    \dontprintsemicolon
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \caption{The (r-Type) ROC-PCA Algorithm}

    \Indentp{-0.5em}
    \Input{Data matrix $\bsbX$; thresholding rule $\Theta(\cdot;\lambda)$; initial estimate $\bsbV_{\perp}^{(0)}$;  nonmonotone line search parameters $\rho$, $\kappa$, $T$ (cf. Section~\ref{sec:vpopt_rocpca} in the text).}
    \Indentp{0.5em} %maximum numbers of outer and inner iterations $M_{outer}$, $M_{inner,1}$, $M_{inner,2}$; error tolerances $\varepsilon_{outer}$, $\varepsilon_{inner,1}$, $\varepsilon_{inner,2}$, $\varepsilon_{inner,3}$;
        \BlankLine
        \emph{Initialization:}\\%$\mathfrak{0}$
        $i \leftarrow 0$, $\bsbV_{\perp}^{(i)} \leftarrow \bsbV_{\perp}^{(0)}$, $\bsbS^{(i)} \leftarrow \bsb{0}$\\



        % \Repeat{$\|\bsbV_{\perp}^{(i)}(\bsbV_{\perp}^{(i)})^T-\bsbV_{\perp}^{(i-1)}(\bsbV_{\perp}^{(i-1)})^T\|_{\infty}/p< \varepsilon_{outer}$  or $i > M_{outer}$}{
        \Repeat{$\|\bsbV_{\perp}^{(i)}(\bsbV_{\perp}^{(i)})^T-\bsbV_{\perp}^{(i-1)}(\bsbV_{\perp}^{(i-1)})^T\|_{\infty}/p$ \text{\upshape is small or} $i$ \text{\upshape is large enough}}{
            \BlankLine
            \emph{$\mathfrak{1}$: $(\bsbmu,\bsbS)$-optimization via $\Theta$-estimation}\\
            $k \leftarrow 0$, $\bar{\bsb{S}}^{(k)} \leftarrow \bsb{S}^{(i)}$\\

            % \emph{$\mathfrak{2.1}$: Optimize $\bsbS$}\\
            % \Repeat{$\|\bar{\bsbS}^{(k)}-\bar{\bsbS}^{(k-1)}\|_{\infty}< \varepsilon_{inner,1}$ or $k > M_{inner,1}$}{
            \Repeat{$\|\bar{\bsbS}^{(k)}-\bar{\bsbS}^{(k-1)}\|_{\infty}$ \text{\upshape is small or} $k$ \text{\upshape is large enough}}{
                $\bar{\bsbS}^{(k+1)} \leftarrow \vec{\Theta}((\bsbI-\frac{1}{n}\bsb{11}^T)\bsbX\bsbV_{\perp}^{(i)}+\frac{1}{n}\bsb{11}^T\bar{\bsbS}^{(k)}); \lambda)$ \label{lineno_thetaEst}\\
                $k \leftarrow k+1$\\
            }
            $\bsb{S}^{(i+1)} \leftarrow \bar{\bsb{S}}^{(k)}$, $\bsb{\mu}^{(i+1)} \leftarrow \frac{1}{n}(\bsbX\bsbV_{\perp}^{(i)}-\bsb{S}^{(i+1)})^T \bsb{1}$\\
            % \emph{$\mathfrak{2.1}$: Update $\bsbmu$}\\
            % $\bsb{\mu}^{(i+1)} \leftarrow \frac{1}{n}(\bsbX\bsbV_{\perp}^{(i)}-\bsb{S}^{(i+1)})^T \bsb{1}$\\


            \BlankLine
            \BlankLine
            \emph{$\mathfrak{2}$: $\bsbVp$-optimization with alternating BB stepsizes and non-monotone line search }\\
            % $f_r \leftarrow +\infty$, $f_* \leftarrow f(\bsbV_{\perp}^{(i)})$, $f_c \leftarrow f(\bsbV_{\perp}^{(i)})$ \\
            $k \leftarrow 0$, $\bar{\bsbV}^{(k)}_{\perp} \leftarrow \bsbV_{\perp}^{(i)}$, $\bsbJ \leftarrow \bsb{1}(\bsbmu^{(i+1)})^{T}+\bsbS^{(i+1)}$, $f^{(0)}\leftarrow \|\bsbX\bar{\bsbV}^{(0)}_{\perp}-\bsbJ\|_F^2$\\%$\bsbG \leftarrow \bsbX^T(\bsbX\bsbV_{\perp}^{(i)}-\bsb{1}(\bsbmu^{(i)})^{T}-\bsbS^{(i)})$
                % \Repeat{$\|\nabla f\|_F< \varepsilon_{inner,2}$ or $\frac{|f^{(k)}-f^{(k-1)}|}{|f^{(k-1)}|}< \varepsilon_{inner,3}$ or $k>M_{inner,2}$}{
                \Repeat{$\|\nabla f\|_F$ \text{\upshape or} $|f^{(k)}-f^{(k-1)}| / |f^{(k-1)}|$ \text{\upshape is small or} $k$ \text{\upshape is large enough}}{
                    \BlankLine
                    \emph{$\mathfrak{2.}$a): BB-update}\\
                    % \lIf{$k=0$}{$\tau \leftarrow 0.5$} \lElse{for even $k$, $\tau \leftarrow \tau_k^0$; otherwise , $\tau \leftarrow \tau_k^1$}
                    If $k=0$, $\tau \leftarrow 0.5$, else $\tau \leftarrow \tau_k^0$ for even $k$, otherwise $\tau \leftarrow \tau_k^1$   (see Section~\ref{sec:vpopt_rocpca})\\
                    % If $k$ is even, $\tau \leftarrow \tau_k^0$ ; otherwise, $\tau \leftarrow \tau_k^1$ (see Section~\ref{sec:vpopt_rocpca} for $\tau_k^0$ and $\tau_k^1$)\\

                    \BlankLine
                    \emph{$\mathfrak{2.}$b): Backtracking} \\
                    $\bsbG \leftarrow \bsbX^T(\bsbX\bar{\bsbV}^{(k)}_{\perp}-\bsbJ)$, $\nabla f \leftarrow \bsbG - \bar{\bsbV}^{(k)}_{\perp} \bsbG^T \bar{\bsbV}^{(k)}_{\perp}$ \\
                    $f_r \leftarrow \max_{0\le j \le \min(k,T)} \{f^{(k-j)}\}$, $f^{\prime} \leftarrow -\frac{1}{2}\|\bsbG(\bar{\bsbV}^{(k)}_{\perp})^T-\bar{\bsbV}^{(k)}_{\perp}\bsbG^T\|_F^2$\\
                    \Repeat{$f^{(k+1)} < f_r +\rho \tau f^{\prime}$}{%f^{\prime}_{\tau}(\bsbV_{\perp}^{(i)})
                        $\widetilde{\bsbV}_{\perp} \leftarrow \bar{\bsbV}^{(k)}_{\perp} - \tau  \bsbA_1 (\bsbI + \tau \bsbA_2^T \bsbA_1/2)^{-1} \bsbA_2^T\bar{\bsbV}^{(k)}_{\perp}$, where $\bsbA_1=[\bsbG$, $\bar{\bsbV}^{(k)}_{\perp}]$ and $\bsbA_2=[\bar{\bsbV}^{(k)}_{\perp}$, $-\bsbG]$\\
                        % $f^{(k+1)} \leftarrow \|\bsbX\widetilde{\bsbV}_{\perp}-\bsb{1}(\bsb{\mu}^{(i+1)})^{T}-\bsb{S}^{(i+1)}\|_F^2$ \\
                        $f^{(k+1)} \leftarrow \|\bsbX\widetilde{\bsbV}_{\perp}-\bsbJ\|_F^2$ \\
                        $\tau \leftarrow \kappa \tau$
                    }
                    % Update $f_r$ according to Section~\ref{sec:vpopt_rocpca}\\%Algorithm~\ref{alg:RefValUpdate}\\
                    $\bar{\bsbV}^{(k+1)}_{\perp} \leftarrow \widetilde{\bsbV}_{\perp}$\\

                %\STATE If $f^{(k+1)}<f_*$, set $f_* \leftarrow f^{(k+1)}$, $f_c\leftarrow f^{(k+1)}$, $t \leftarrow 0$;
               % otherwise, set $f_c \leftarrow \max(f_c,f^{(k+1)})$, $t \leftarrow t+1$, and if $t=T$, set $f_r \leftarrow f_c$, $f_c \leftarrow f^{(k+1)}$, $t \leftarrow 0$

                    $k \leftarrow k+1$\\
                }

            $\bsbV_{\perp}^{(i+1)} \leftarrow \bar{\bsbV}^{(k)}_{\perp}$\\
            $i \leftarrow i+1$\\
            \BlankLine

        }
    \BlankLine
    \Indentp{-0.5em}
    \Output{$\hat{\bsb{V}}_{\perp}=\bsbV_{\perp}^{(i)}$, $\hat{\bsb{S}}=\bsb{S}^{(i)}$ and $\hat{\bsb{\mu}}=\bsb{\mu}^{(i)}$}

\end{algorithm}
% \DecMargin{1.5em}

